MMT: Mutation Testing of Java Bytecode with Model Transformation -- An Illustrative Demonstration

Mutation testing is an approach to check the robustness of test suites. The program code is slightly changed by mutations to inject errors. A test suite is robust enough if it finds such errors. Tools for mutation testing usually integrate sets of mutation operators such as, for example, swapping arithmetic operators; modern tools typically work with compiled code such as Java bytecode. In this case, the mutations must be defined in such a way that the mutated program still can be loaded and executed. The results of mutation tests depend directly on the possible mutations. More advanced mutations and even domain-specific mutations can pose another challenge to the test suite. Since extending the classical approaches to more complex mutations is not well supported and is difficult, we propose a model-driven approach where mutations of Java bytecode can be flexibly defined by model transformation. The corresponding tool called MMT has been extended with advanced mutation operators for modifying object-oriented structures, Java-specific properties and method calls of APIs, making it the only mutation testing tool for Java bytecode that supports such mutations.

==> 2_example.tex <==
% !TeX spellcheck = en_US
\section{Introductory example}
\label{sec:example}


A simple example for class-level Java bytecode mutation is the deletion of an overriding method.
In Fig.~\ref{fig:concreteMutation} a snippet of a Java bytecode example is shown, before and after a mutation.  
In this example, the class \texttt{Child} extends the class \texttt{Parent} and overrides method \texttt{printY()}.
To test the robustness of an associated test suite, this code can be mutated by deleting exactly this overriding method. 
The resulting bytecode model is shown on the right of Fig.~\ref{fig:concreteMutation}.
As an effect,  the method \texttt{printY()} does not print the variable \texttt{y} of class \texttt{Child} (where it is set to \verb!"Child"!) but of class \texttt{Parent} (where it is set to \verb!"Parent"!). 

The figure also shows two test cases at the bottom right, one of which, namely \texttt{testStrong}, would detect this mutation:
While the test succeeds before the mutation, it fails afterwards.
The second test, \texttt{testWeak}, would not detect the mutation, as both before and after the mutation, the condition that a non-empty String is returned holds.

To get a syntactically correct program after mutation, a mutation operator that deletes overriding methods has to ensure that it does not delete constructors. 
However, all instructions in the method to be deleted also have to be deleted as well. 

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{./Figures/ConcreteMutation.png}%
\caption{Java bytecode model before (left) and after (right) deleting the overriding method \texttt{printY()}. The test at the bottom right succeeds before and fails after the mutation.}%
\label{fig:concreteMutation}
\end{figure}



==> 5_evaluation.tex <==
% !TeX spellcheck = en_US
\section{Evaluation}
\label{sec:evaluation}
We evaluated MMT with respect to the following research questions:

\begin{enumerate}
\item Which mutation operators does MMT offer compared to other mutation testing tools?
%\item How powerful is MMT in specifying mutation operators compared to other mutation testing tools? 
%What kinds of mutation operators can be specified, cannot be specified?
\item How efficacious is MMT compared to other mutation testing tools? 
%With respect to simple Java projects (mutating only arithmetic operations) and more object-oriented projects? 
%\gt{Choose at least two projects, e.g., the project on matrix operations (https://github.com/soursop/functional-matrix-operator) and the simple OO-project.}
\item How efficient is MMT compared to other mutation testing tools? 
%\gt{Only for one or more simple project(s).}
\end{enumerate}

To answer the questions, we compared our tool MMT with three different mutation testing tools for Java source code or bytecode, namely Mujava~\cite{MOK06}, Jumble~\cite{IPT+07},  and Pitclipse~\cite{CLH+16}. 
All evaluation data are available at \url{https://gitlab.uni-marburg.de/fb12/plt/modbeam-mt/mmt/-/tree/main/benchmarks}
Note that we evaluate the {\em efficacy} of MMT and other mutation testing tools instead of the {\em effectiveness},  since we evaluate them on small and partly artificial Java projects.  For evaluating their effectiveness, we would apply mutation testing to larger, real-world Java projects. 

%\cb{Java version of ModBEAM/MMT. Should we leave this in? ...If so, maybe better in Sec. \ref{sec:modbeam}? Maybe some (in particular invokedynamic) can be easily fixed}
%
%Out tool MMT uses the ModBEAM meta-model of Java bytecode and therefore is limited to projects written in a supported Java version.
%In fact, the ModBEAM meta-model and its Eclipse plug-in do not name a specific Java version but they can in principle operate on any Java code, whereby a few language features are currently not supported or buggy: 
%\begin{itemize}
%\item final variables in try-with-resources 
%\item switch Expressions
%\item the invokedynamic instruction (used for \lstinline[language=java]!MethodHandle!, record classes and may be used for String concatenation).
%\end{itemize}

%
%\gt{ Here a table with tool characteristics such as Java/Java bytecode, Java version of test project, input-output
%}

%\begin{table}
%	\caption{Mutation testing tools - Characteristics}
%	\label{tab:tools}
%%	\footnotesize
%	\centering
%	\begin{tabular}{lcccc}
%		\toprule
%		\textbf{Tool name} & \textbf{Bytecode} & \textbf{Java version} & \textbf{Input} & \textbf{Output}\\
%		\midrule
%		MMT & x &  ? &  &\\
%		Pitclipse & &&  &\\
%		Jumble &  &  &&\\
%		Mujava&  & & &\\
%		\bottomrule
%	\end{tabular}
%\end{table}
%


\subsection{Comparison with respect to available mutation operators}
%\gt{We should add information about the specification mechanisms for mutation operators in Pitclipse, Jumble and Mujava. }
While Pitclipse and Jumble use only basic mutation operators, MMT and Mujava also use class-level operators.  
It is noticeable that Jumble provides a high number of arithmetic operators.
%In fact, all 56 operators in Jumble are covered by only 21 operators in Pitclipse.  
%\cb{Should this be 51?  ...  Can we explain how this is possible?}
%\gt{Jetzt klar?}
MMT and Mujava have many operators in common.
In addition to arithmetic, relational, and conditional operators, both also share many operators for changing the class structure.
MMT is the only mutation testing tool for Java bytecode that supports class-level operators, and the only one of these three tools that also includes operators for mutating Java Collection Framework method calls.
So far, MMT does not provide operators that modify return values, variables and constant values. 
However, these operators are easy to specify and will be added in the near future. 
See Table~\ref{tab:MutationOperatorPerTool} for an overview of the number of mutation operators in each operator category and tool.



\begin{table}
	\caption{Number of mutation operators in different operator categories and tool}
	\label{tab:MutationOperatorPerTool}
%	\footnotesize
	\centering
	\begin{tabular}{lcccc}
		\toprule
		\textbf{Mutation operator category} & \textbf{MMT} & \textbf{Pitclipse} & \textbf{Jumble} & \textbf{Mujava}\\
		\midrule
		Arithmetic operators & 12 &  9 & 32 &7\\
		Relational  \&  conditional operators & 14 & 16 & 1 &7\\
		Inheritance operators & 8 & 0 &0& 8\\
		Polymorphism operators& 12 & 6 & 1 &12\\
		Return values operators & 0 & 6 & 5 &0\\
		Variable \& constants operators & 0 & 14 & 17 & 3\\
		Java-specific operators & 6 & 0 & 0 &10\\
		Collection operators & 6 & 0 &0 &0\\
		\midrule
		\textbf{Total}& \textbf{56} & \textbf{51} & \textbf{56} & \textbf{47} \\
		\bottomrule
	\end{tabular}
\end{table}



%\begin{figure}
%\centering
%\includegraphics[width=\columnwidth]{figures/MutationOperatorPerTool.png}%
%\caption{}%
%\label{fig:MutationOperatorPerTool}
%\end{figure}

%\gt{Looking at the number of mutants generated for all 5 Java projects,  we  found that Pitclipse in particular performed a high number of mutations on arithmetic operators, which are very simple. 
%MMT has generated the fewest mutants, but its mutation score is only slightly worse than the scores of the other tools. 
%On the other hand, Pitclipse generated the highest number of mutants, but achieved an even slightly worse mutation score than MMT. 
%See Fig.~\ref{fig:MutantNumber} for an overview of the number of mutants that have been generated per operator. 
%Fig.~\ref{fig:MutationScore} shows the numbers of mutants, living or killed, and the resulting mutation scores for all sample projects together. 
%The mutation score of MMT only for the custom project is 0,91, which is quite high.}
%

%\gt{Figures are just for orientation, they will be replaced.}
%
%\begin{figure}
%\centering
%\includegraphics[width=\columnwidth]{figures/MutantNumber.png}%
%\caption{}%
%\label{fig:MutantNumber}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=\columnwidth]{figures/MutationScore.png}%
%\caption{}%
%\label{fig:MutationScore}
%\end{figure}

\subsection{Comparison with respect to efficacy and efficiency of mutation testing}

To evaluate the efficacy and efficiency of the four tools, we selected 5 small Java projects, 4 of which mainly perform computations in one class and use almost no object-oriented concepts. 
This is due to the fact that Jumble and PITclipse do not support the mutation of program structures, Java-specific features, and collection method calls. 
Only one of the Java projects, is slightly larger and uses truly object-oriented concepts. 
Concretely, we used the projects Cal, TestPat, TrashAndTakeOut from \cite{AO16}, the project triangle-example from \cite{Triangle}, and a custom project we developed to test all object-oriented, Java-specific and collection-specific mutation operators we specified in MMT.
Table~\ref{tab:JavaProjects} shows key values about the size of each project. 

\begin{table}
	\caption{Java projects used for evaluation - key values}
	\label{tab:JavaProjects}
%	\footnotesize
	\centering
	\begin{tabular}{lcccc}
		\toprule
		\textbf{Project name} & \textbf{Classes} & \textbf{Methods} & \textbf{Lines of code} & \textbf{Number of tests}\\
		\midrule
		Cal & 1 &  1 & 20 &11\\
		TestPat  & 1 & 1 & 33 &15\\
		TrashAndTakeOut & 1 & 2 &25& 9\\
		triangle-example& 1 & 2 & 45 &12\\
		Custom project & 8& 48 & 270 &15\\
		\bottomrule
	\end{tabular}
\end{table}


To compare the efficacy of the mutation testing tools, the tools should find mutants for which there are no tests in the test suite that can kill them.  These mutants are referred to as {\em effective}. 
Unfortunately, none of the tools considered report on the effectiveness of the mutants generated. 
There are also no benchmarks for generating effective mutants. 
Therefore, for now, we calculated the mutation scores for the selected Java projects and for each tool, as is common practice in evaluations of other mutation testing tools such as  \cite{schuler2009javalanche,Jus14,GGLM21}.
Additional means for comparing the effectiveness of mutation testing tools should be developed in the future.
%\gt{Hier auf das Problem mit dem Mutation Score eingegangen. Ist das ueberzeugend?}
%\gt{Why is it a good idea to use the mutation score?}

In Table~\ref{tab:ScoreAndRuntime}, all mutation scores are listed.  
%We see that MMT has the highest mutation scores for the projects Cal and triangle, the mutation score of Mujava dominates for TestPat and TrashAndTakeOut,  and Jumble has the highest mutation score for the custom project. 
In general,  the mutation scores of the tools vary across the projects and MMT is comparable to existing mutation testing tools in terms of mutation scores.
As the mutation score only indicates how many mutants could be killed, it remains open which mutation operators were applied  at which location in the code.  
(More details can be found in the evaluation data.)
It is a task of future work, to further investigate how effective these tools are in measuring the robustness of a test suite.

To compare the efficiency of the mutation testing tools,  we measured the runtime that the tools required for the selected Java projects. 
For each project, the measured times include the time to generate the mutants and to run the test suite on each of them. 
Table~\ref{tab:ScoreAndRuntime} also shows the runtime for all projects.  
%MMT is the fastest tool for Cal and TestPat; for TrashAndTakeOut, triangle, and the custom project PITclipse was the fastest tool. 
So also in terms of the runtime, MMT is comparable to existing mutation tools. 
% in der gleichen Groessenordnung dabei
%\cb{Yes, but the perform fewer mutations. Since the mutation score is not a good indicator for  the accuracy, it is also not fully correct to say that we take the same time to achieve the same result by requiring slower but fewer steps.}

%\gt{For the custom project we have the following number of mutants per kind of mutation operators applied:\\
%MMT: 15 with inheritance operators, 12 with Java/specific, 13 with collection operators, 2 with traditional operators\\
%Jumble: 10 constant operators, 14 return value o. , 18 assignment o. , 12 method call o. , 1 arithmetic o., altogether 54 with traditional o. \\
%Mujava: 164 with traditional o. , 93 with structural o. \\
%Pitclipse: 29 return value, 19 empty return, 47 method call, 19 negation36 constant replacement, altogether 282 with traditional o. \\
%Do we have mutants that others tools do not have?
%In MMT the container test cannot kill mutants where collection operators were applied.
%}

\begin{table}
	\caption{Mutation testing of Java projects - Mutation score and runtime
	}
	\label{tab:ScoreAndRuntime}
%	\footnotesize
	\centering
	\begin{tabular}{lrrrrr}
		\toprule
		\textbf{Tool /Project name} & \textbf{Cal} & \textbf{TestPat} & \textbf{TrashAnd...} & \textbf{triangle} & \textbf{Custom project}\\
		\midrule
		MMT - mutation score& 0.77 &  0.57 & 0.67 & 1.00 & 0.45\\
		PITclipse - mutation score & 0.51& 0.81& 0.81 &0.79 & 0.43\\	
		Jumble - mutation score & 0.63 & 0.93&0.80& 0.97 & 0.50 \\	
		mujava- mutation score & 0.70 &0.96 &0.86 &0.83 & 0.33\\
		\midrule
		MMT- runtime & 12.6&  6. 8& 8.3 &16.0 & 38.0\\
		PITclipse	- runtime & 31.0&  52.0 & 5.0 &10.0& 4.0\\	
		Jumble - runtime & 28.5 &  13.3 & 13.7 &16.0 & 22.0\\
		mujava - runtime & 84.0 &  >600.0 & 10.5 &15.0 & 12.0\\	
		\bottomrule
	\end{tabular}
\end{table}

\subsection{Threats to validity}

The selection of mutation testing tools is representative as the established tools Jumble, PITclipse and Mujava are considered, however, the mutation testing tools Major~\cite{Jus14} and Javalanche~\cite{schuler2009javalanche} should also be considered for comparison, as they also can mutate Java bytecode. 
A quick check of their mutation operators revealed that they also do not support structural mutation operators.
A deeper comparison with Major and Javalanche is planned for future work. 

The Java projects selected for evaluating efficacy and efficiency are computa\-tion-oriented as Jumble and PITclipse do not have structure-oriented mutation operators, and moreover, the projects are quite small.   The custom project shows more class structure; it is handy for evaluating structure-oriented operators, but it is an artificial project and also quite small.  
A comparison using larger, real-world projects is planned for future work. 

A mutation testing tool is effective if it generates program mutants that find missing tests in the test suite.
The mutation score does not really reflect this. 
A mutation score of 1.0 simply states that all mutants generated could be killed.
However, if the program was  modified differently, a mutant could occur that could not be killed. %and missing tests could be found in the test suite. 
Therefore,  achieving a mutation score of 1.0 does not automatically mean that a mutation testing tool is sufficient, instead it may be the case, that it may simply have generated mutants that are trivial to detect. 
%\cb{Rewrote this sentence. Is it correct and clearer?}
It is only good if the tests in the test suite actually cover the full code.
%\cb{The meaning of ``no missing tests'' is uncIear. I think it should say ``if the tests in the test suite actually cover the full code'' -- is  that what you want to say here?}
MMT can provide a wide range of mutation operators, which can be considered as a good prerequisite for generating diverse mutants, and therefore, generating mutants that are not killed by the test suite.
%A mutation score lower than 1.0 means that some mutants could not be killed; the question here is whether the mutants found all point to different kinds of missing tests in the test suite, which is desirable. 
Future evaluations should replace the mutation score as a measure for efficacy with another score that more clearly demonstrates efficacy.



==> 5_evaluationNew.tex <==
% !TeX spellcheck = en_US
\section{Initial evaluation}
\label{sec:evaluation}
We have evaluated MMT with respect to the following research questions:

\begin{enumerate}
\item Which mutation operators does MMT offer compared to other mutation testing tools?
\item Which information does MMT provide compared to other mutation testing tools?
\end{enumerate}

\subsection{Comparison of mutation operator sets}
\gt{We compare the mutation operator set of MMT with the operator sets of other mutaion testing tools such as Major and PITest. It should become clear that MMT offers not only the basic operators supported by all mutation testing tools, but also more advanced operators. And MMT even allows to specify new operators with Henshin. (Shall we include how this is done?)}

Major offers a variety of operator replacements. This set includes replacements of arithmetic, conditional, logical, relational,  and shift operators. In addition, unary and literal operators can be replaced and expressions can be replaced with default values.  Moreover,  single statements can be deleted. 

PITest offers the following operators: Replacements of conditionals,  arithmetic, logical, shift, unary operators, literals, 
In addition, exchange of increment with decrement, return values, condition with true or false, constructor call with null, method call with some literal of the return type,  and deletion of method calls. 

\subsection{Comparison of output information}
\gt{We compare the output of MMT with the output by other mutation testing tools.  MMT is the only tool with a GUI? (Except of WODEL/Test)}

Major: 
Mutants’ unique number (id), Name of the applied mutation operator, Original operator symbol, Replacement operator symbol, Fully qualified name of the mutated method, Line number in original source file, Summary of the applied transformation (<from> |==> <to>), export of source code mutants, enabling/disabling of mutation operators





==> bibliography.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{offutt2001mutation}
A.~J. Offutt and R.~H. Untch, ``Mutation 2000: Uniting the orthogonal,''
  \emph{Mutation testing for the new century}, pp. 34--44, 2001.

\bibitem{Nystrom2003}
\BIBentryALTinterwordspacing
N.~Nystrom, M.~R. Clarkson, and A.~C. Myers, ``Polyglot: An extensible compiler
  framework for java,'' in \emph{Compiler Construction}.\hskip 1em plus 0.5em
  minus 0.4em\relax Springer, 2003, pp. 138--152. [Online]. Available:
  \url{https://doi.org/10.1007/3-540-36579-6\_11}
\BIBentrySTDinterwordspacing

\bibitem{asm}
\BIBentryALTinterwordspacing
E.~Bruneton, R.~Lenglet, and T.~Coupaye, ``{ASM}: a code manipulation tool to
  implement adaptable systems,'' \emph{Adaptable and extensible component
  systems}, vol.~30, p.~19, 2002. [Online]. Available:
  \url{http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.117.5769}
\BIBentrySTDinterwordspacing

\bibitem{bcel}
``The {BCEL} homepage,'' \url{https://commons.apache.org/proper/commons-bcel/},
  May 2022, accessed: October 10, 2022.

\bibitem{Jus14}
R.~Just, ``The major mutation framework: Efficient and scalable mutation
  analysis for java,'' in \emph{Proc. of the 2014 Int. Symp. on Software
  Testing and Analysis}, 2014, pp. 433--436.

\bibitem{schuler2009javalanche}
D.~Schuler and A.~Zeller, ``Javalanche: Efficient mutation testing for java,''
  in \emph{Proc. of the 7th Joint Meeting of the European Software Engineering
  Conference and the ACM SIGSOFT Symposium on The Foundations of Software
  Engineering}, 2009, pp. 297--298.

\bibitem{CLH+16}
H.~Coles, T.~Laurent, C.~Henard, M.~Papadakis, and A.~Ventresque, ``Pit: a
  practical mutation testing tool for java,'' in \emph{Proc. of the 25th Int.
  Symp. on Software Testing and Analysis}, 2016, pp. 449--452.

\bibitem{BTNW20}
\BIBentryALTinterwordspacing
C.~Bockisch, G.~Taentzer, N.~Nassar, and L.~Wydra, ``Java bytecode verification
  with {OCL}: Why, how and when,'' \emph{J. Object Technol.}, vol.~19, no.~3,
  pp. 3:1--16, 2020. [Online]. Available:
  \url{https://doi.org/10.5381/jot.2020.19.3.a13}
\BIBentrySTDinterwordspacing

\bibitem{YBRA17}
\BIBentryALTinterwordspacing
B.~M. Yildiz, C.~Bockisch, A.~Rensink, and M.~Aksit, ``An {MDE} approach for
  modular program analyses,'' in \emph{Companion to the 1st Int. Conf. on the
  Art, Science and Engineering of Programming}, J.~B. Sartor, T.~D'Hondt, and
  W.~D. Meuter, Eds.\hskip 1em plus 0.5em minus 0.4em\relax {ACM}, 2017, pp.
  15:1--15:5. [Online]. Available:
  \url{https://doi.org/10.1145/3079368.3079392}
\BIBentrySTDinterwordspacing

\bibitem{ABJKT10}
\BIBentryALTinterwordspacing
T.~Arendt, E.~Biermann, S.~Jurack, C.~Krause, and G.~Taentzer, ``{Henshin:
  Advanced Concepts and Tools for In-Place EMF Model Transformations},'' in
  \emph{Proc.\ MODELS}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2010,
  pp. 121--135. [Online]. Available: \url{https://www.eclipse.org/henshin}
\BIBentrySTDinterwordspacing

\bibitem{emfWebsite}
``Eclipse {M}odeling {F}ramework website,''
  \url{https://www.eclipse.org/modeling/emf/}, Apr. 2016.

\bibitem{OMG14}
``{Object Constraint Language, Version 2.4, Object Management Group},''
  http://www.omg.org/spec/OCL/2.4, {Object Management Group}, 2014.

\bibitem{OMK06}
\BIBentryALTinterwordspacing
J.~Offutt, Y.-S. Ma, and Y.-R. Kwon, ``The class-level mutants of mujava,'' in
  \emph{Proceedings of the 2006 International Workshop on Automation of
  Software Test}, ser. AST '06.\hskip 1em plus 0.5em minus 0.4em\relax ACM,
  2006, p. 78–84. [Online]. Available:
  \url{https://doi.org/10.1145/1138929.1138945}
\BIBentrySTDinterwordspacing

\bibitem{BET12}
\BIBentryALTinterwordspacing
E.~Biermann, C.~Ermel, and G.~Taentzer, ``Formal foundation of consistent {EMF}
  model transformations by algebraic graph transformation,'' \emph{Softw. Syst.
  Model.}, vol.~11, no.~2, pp. 227--250, 2012. [Online]. Available:
  \url{https://doi.org/10.1007/s10270-011-0199-7}
\BIBentrySTDinterwordspacing

\bibitem{NassarKAT18}
\BIBentryALTinterwordspacing
N.~Nassar, J.~Kosiol, T.~Arendt, and G.~Taentzer, ``{OCL2AC:} automatic
  translation of {OCL} constraints to graph constraints and application
  conditions for transformation rules,'' in \emph{Graph Transformation - 11th
  International Conference, {ICGT} 2018, Proceedings}, ser. LNCS, vol.
  10887.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2018, pp. 171--177.
  [Online]. Available: \url{https://doi.org/10.1007/978-3-319-92991-0\_11}
\BIBentrySTDinterwordspacing

\bibitem{IPT+07}
S.~A. Irvine, T.~Pavlinic, L.~Trigg, J.~G. Cleary, S.~Inglis, and M.~Utting,
  ``Jumble: Java byte code to measure the effectiveness of unit tests,'' in
  \emph{Testing: Academic and Industrial Conference Practice and Research
  Techniques}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2007, pp. 169--175.

\bibitem{littledarwin}
A.~Parsai, A.~Murgia, and S.~Demeyer, ``{LittleDarwin: a feature-rich and
  extensible mutation testing framework for large and complex Java systems},''
  in \emph{Int. Conf. on Fundamentals of Software Engineering}.\hskip 1em plus
  0.5em minus 0.4em\relax Springer, 2017, pp. 148--163.

\bibitem{MBT06}
J.-M. Mottu, B.~Baudry, and Y.~L. Traon, ``Mutation analysis testing for model
  transformations,'' in \emph{Europ. Conf. on Model Driven
  Architecture-Foundations and Applications}.\hskip 1em plus 0.5em minus
  0.4em\relax Springer, 2006, pp. 376--390.

\bibitem{GGLM21}
\BIBentryALTinterwordspacing
P.~G{\'{o}}mez{-}Abajo, E.~Guerra, J.~de~Lara, and M.~G. Merayo, ``Wodel-test:
  a model-based framework for language-independent mutation testing,''
  \emph{Softw. Syst. Model.}, vol.~20, no.~3, pp. 767--793, 2021. [Online].
  Available: \url{https://doi.org/10.1007/s10270-020-00827-0}
\BIBentrySTDinterwordspacing

\end{thebibliography}

